New Characterizations of Core Imputations of Matching and $b$-Matching Games

We give new characterizations of core imputations for the following games: * The assignment game. * Concurrent games, i.e., general graph matching games having non-empty core. * The unconstrained bipartite $b$-matching game (edges can be matched multiple times). * The constrained bipartite $b$-matching game (edges can be matched at most once). The classic paper of Shapley and Shubik \cite{Shapley1971assignment} showed that core imputations of the assignment game are precisely optimal solutions to the dual of the LP-relaxation of the game. Building on this, Deng et al. \cite{Deng1999algorithms} gave a general framework which yields analogous characterizations for several fundamental combinatorial games. Interestingly enough, their framework does not apply to the last two games stated above. In turn, we show that some of the core imputations of these games correspond to optimal dual solutions and others do not. This leads to the tantalizing question of understanding the origins of the latter. We also present new characterizations of the profits accrued by agents and teams in core imputations of the first two games. Our characterization for the first game is stronger than that for the second; the underlying reason is that the characterization of vertices of the Birkhoff polytope is stronger than that of the Balinski polytope.

==> Edges2.tex <==


\subsection{The second issue: Allocations made to teams by core imputations}
\label{sec.edges}

\begin{proof}
The proof is similar to that of Theorem \ref{thm.vertices}. Let $x$ and $y$ be optimal solutions to LP (\ref{eq.core-primal-bipartite}) and LP (\ref{eq.core-dual-bipartite}), respectively. By the Complementary Slackness Theorem, for each $e = (u, v) \in E: \ \ x_e \cdot (y_u + y_v - w_e) = 0$.

We will prove the reverse direction of the implication first. Suppose $e$ is viable or essential. Then there is an optimal solution to the primal, say $x$, under which it is matched. Therefore,  $x_e > 0$. Let $y$ be an arbitrary optimal dual solution. Then, by the Complementary Slackness Theorem, $y_u + y_v = w_e$, i.e., $e$ is fairly paid in $y$. Varying $y$ over all optimal dual solutions, we get that $e$ is always paid fairly. 

To prove the forward direction, we will use strict complementarity. It implies that corresponding to each team $e$, there is a pair of optimal primal and dual solutions $x$ and $y$ such that either $x_e = 0$ or $y_u + y_v = w_e$ but not both. 

Assume that team $e$ is always fairly paid, i.e., under every optimal dual solution $y$, $y_u + y_v = w_e$. By strict complementarity, there must be an optimal primal solution $x$ for which $x_e > 0$. Since the polytope defined by the constraints of the primal LP (\ref{eq.core-primal-bipartite}) has integral optimal vertices, $x$ is a convex combination of optimal assignments. Therefore, there must be an optimal assignment in which $e$ is matched. Therefore $e$ is viable or essential and the forward direction also holds. 
\end{proof}


Negating both sides of the implication proved in Theorem \ref{thm.edges}, we get the following  implication. For every team $e \in E$: 
		\[ e \ \mbox{is subpar} \ \iff \ e \ \mbox{is sometimes overpaid} \]

Clearly, this statement is equivalent to the statement proved Theorem \ref{thm.edges} and hence contains no new information. However, it provides a new viewpoint. These two equivalent  statements yield the following assertion, which at first sight seems incongruous with what we desire from the notion of the core and the just manner in which it allocates profits:

\begin{center}
{\em Whereas viable and essential teams are always paid fairly, subpar teams are sometimes overpaid.}
\end{center}


How can the core favor subpar teams over viable and essential teams? An explanation is provided in the Introduction, namely a subpar team $(i, j)$ gets overpaid because $i$ and $j$ create worth by playing in competent teams with other players. 

Finally, we observe that contrary to Corollary \ref{cor.vertices}, which says that the set of essential players is non-empty, the set of essential teams may be empty, as is the case in Examples \ref{ex.1} and \ref{ex.2} in Section \ref{sec.negotiation}.  


%{\bf 3).} Clearly the worth of the game is generated by teams that do play. Assume that $(u, v)$ is such a team in an optimal assignment. Since $x_{uv} > 0$, by complementary slackness we get that $y_u + y_v = w_{uv}$, where $y$ is a core imputation. Thus core imputations distribute the worth generated by a team among its players only. In contrast, the ${2 \over 3}$-approximate core imputation for the general graph matching game given in \cite{Va.general} distributes the worth generated by teams which play to non-playing agents as well, thereby making a more thorough use of the TU aspect.   

\subsection{The third issue: Degeneracy}
\label{sec.degeneracy}

 Next we use Theorems \ref{thm.vertices} and \ref{thm.edges} to get insights into degeneracy. Clearly, if an assignment game is non-degenerate, then every team and every player is either always matched or always unmatched in the set of maximum weight matchings in $G$, i.e., there are no viable teams or players. Since viable teams and players arise due to degeneracy, in order to understand the phenomenon of degeneracy, we need to understand how viable teams and players behave with respect to core imputations; this is done in the next corollary.
 
\begin{corollary}
	\label{cor.degen}
	In the presence of degeneracy, imputations in the core of an assignment game treat:
	\begin{itemize}
			\item  viable players in the same way as subpar players, namely they are never paid.  
		\item viable teams in the same way as essential teams, namely they are always fairly paid. 
	\end{itemize}
\end{corollary}


 
 

















==> talk.tex <==
\section{Talk}
\label{sec.talk}


New Insights into a Half-Century-Old Work: the Core of the Matching Game


\bigskip

The classic 1971 paper of Shapley and Shubik characterized the core of the assignment game using ideas from matching theory and LP-duality theory and their highly non-trivial interplay. 

The core is a quintessential solution concept in cooperative game theory --- it contains all ways of distributing the total worth of a game among agents in such a way that no sub-coalition has incentive to secede from the grand coalition. Additionally, the pristine structural properties of the assignment game make it a paradigmatic setting for studying the intricacies of this solution concept, with a view to tackling profit-sharing in real-life situations. 

We build on the Shapley-Shubik work in two ways: 

1). We study core imputations of the assignment game through the lens of complementarity, thereby obtaining a relationship between the competitiveness of individuals and teams of agents and the amount of profit they accrue. 

2). Whereas the core of the assignment game is always non-empty, that of the general graph matching game can be empty. We show how to salvage the situation via the notion of approximate core.

 
This talk is completely self-contained. It is based on:

https://www.sciencedirect.com/science/article/pii/S0899825622000239?via%3Dihub

https://arxiv.org/pdf/2202.00619.pdf




\newpage


LP-Duality Theory and the Cores of Games


The core is a quintessential solution concept in cooperative game theory and LP-duality theory has played a central role in its study, right from its early days to the present time. The classic 1971 paper of Shapley and Shubik showed the ``right'' way of exploiting this theory --- in the context of characterizing the core of the assignment game. 

The LP-relaxation of this game  has the following key property: the polytope defined by its constraints has integral vertices; in this case, they are matchings in the underlying graph. Similar characterizations for several basic combinatorial optimization games followed; throughout, this property was established by showing that the underlying linear system is totally unimodular (TUM). 

We will first exploit TUM further via a very general formulation due to Hoffman and Kruskal (1956). The way take this methodology to its logical next step is to use total dual integrality (TDI). In the process, we address new classes of games which have their origins in two major theories within combinatorial optimization, namely perfect graphs and polymatroids.

Whereas the core of the assignment game is always non-empty, that of the general graph matching game can be empty. We show how to salvage the situation --- again using LP-duality in a fundamental way. 








